Manifold DivideMix: A Semi-Supervised Contrastive Learning Framework for Severe Label Noise

Deep neural networks have proven to be highly effective when large amounts of data with clean labels are available. However, their performance degrades when training data contains noisy labels, leading to poor generalization on the test set. Real-world datasets contain noisy label samples that either have similar visual semantics to other classes (in-distribution) or have no semantic relevance to any class (out-of-distribution) in the dataset. Most state-of-the-art methods leverage ID labeled noisy samples as unlabeled data for semi-supervised learning, but OOD labeled noisy samples cannot be used in this way because they do not belong to any class within the dataset. Hence, in this paper, we propose incorporating the information from all the training data by leveraging the benefits of self-supervised training. Our method aims to extract a meaningful and generalizable embedding space for each sample regardless of its label. Then, we employ a simple yet effective K-nearest neighbor method to remove portions of out-of-distribution samples. By discarding these samples, we propose an iterative "Manifold DivideMix" algorithm to find clean and noisy samples, and train our model in a semi-supervised way. In addition, we propose "MixEMatch", a new algorithm for the semi-supervised step that involves mixup augmentation at the input and final hidden representations of the model. This will extract better representations by interpolating both in the input and manifold spaces. Extensive experiments on multiple synthetic-noise image benchmarks and real-world web-crawled datasets demonstrate the effectiveness of our proposed framework. Code is available at https://github.com/Fahim-F/ManifoldDivideMix.

==> algorithms/ManifoldDivideMix.tex <==
\begin{algorithm*}
    \caption{Manifold DivideMix}
    
    \label{alg:manifold}
    
    \begin{algorithmic}[1]
        \Require $\theta, \psi, \phi$ \Comment{Backbone, Projection head and classification head parameters}
        \Require $(\mathcal{X}, \mathcal{Y})$ \Comment{Training Data}
        \Require $\lambda_u, \lambda_c$ \Comment{Unsupervised and contrastive loss weights}
        \Require $k$, $initRemoval$, $p$ \Comment{Parameter of KNN, constant ratio for OOD removal, percentage of removal}
        \Require $\tau_2$, $\alpha$ \Comment{GMM threshold, Parameter of $\betadist$ distribution for Mixup}
        % \Require $\betadist$ \Comment{distribution parameter $\alpha$ for Mixup}
        
        % \Ensure output

        \Statex

         \State $\theta,  \psi \gets \text{SSLModel}(\mathcal{X}, \theta,  \psi)$
         
            \Statex
            
         \State  $\text{OODScore} \gets  \text{KNN}(\mathcal{X}, \theta, \phi, k)$   \Comment{Compute OOD score based on the average distance of k-nearest neighbors}
                   
          \State $\text{RemovalRate} \gets initRemoval $   \Comment{ Initial sample removal rate}

          \State   $\text{OODMask} \gets \text{TopScore}(OODScore, RemovalRate) $  \Comment{Select samples with highest OOD score  to discard them}
          
            \Statex
            
          \State $(\theta,  \phi) \gets \text{ Warmup}(\mathcal{X}, \mathcal{Y},  \theta,  \phi, \text{OODMask})$   \Comment{Warmup training of $f_2$ and fine-tuning of $f_1$}
         
            \Statex     

        \While{$e \leq $ MaxEpoch / $10$ }
        
            \Statex
              
         \State  $ OODScore \gets  \text{KNN}(\mathcal{X}, \theta, \phi, k)$   \Comment{Compute OOD score based on the average distance of k-nearest neighbors}
            
          \State $ RemovalRate \gets RemovalRate + p $   \Comment{ Compute percentage of sample removal}
            
           \State   $\text{OODMask} \gets TopScore(OODScore, RemovalRate) $  \Comment{Select samples with highest OOD score  to discard them}
           
           \State   $ \mathcal{W} \gets \text{GMM}( \mathcal{X}, \mathcal{Y}, \theta, \phi, \text{OODMask} ) $  \Comment{Model per-sample loss distribution to obtain clean probability}
           
            \Statex        
                       
            \For{$ iter \gets 1$ \textbf{to} $10$}
            
            \Statex
            
                \State $\mathcal{X}  \gets  \{ (\mathbf{x}_i,\mathbf{y}_i, w_i) : w_i=p \left ( x_i=\text{clean} | \ell^{sup} , \gamma ) \ge \tau_2  ,  \forall (x_i,y_i,w_i) \in (\mathcal{X},\mathcal{Y},\mathcal{W})\right \}$ \Comment{Construct labeled set}
                
                \State $\mathcal{U}  \gets  \{ (\mathbf{x}_i,\mathbf{y}_i, w_i) : w_i=p \left ( x_i=\text{clean} | \ell^{sup} , \gamma ) < \tau_2, \forall (x_i,w_i) \in (\mathcal{X},\mathcal{W})\right \}$ \Comment{Construct unlabeled set}
                
            \Statex    
            
                \State $ ( \mathcal{X}^\prime, \mathcal{U}^\prime, \mathcal{H}_x^\prime, \mathcal{H}_u^\prime) \gets \text{MixEMatch} (\mathcal{X}, \mathcal{U}, \theta, \phi, \T, \alpha) $  \Comment{Apply MixEMatch Algorithm}
                
            \Statex
                 
                \State $\mathcal{L}^{semi} \gets \mathcal{L}^{sup} + \lambda_u \mathcal{L}^{unsup} + \lambda_c \mathcal{L}^{self} $ \Comment{Compute total loss}
                
                \State $\theta, \phi = SGD(\mathcal{L}^{semi}, \theta, \phi) $ \Comment{Update model parameters}
            \EndFor
        \EndWhile

       
    \end{algorithmic}
\end{algorithm*} 


==> algorithms/mixematch.tex <==
\begin{algorithm}
    \caption{MixEMatch}
    
    \label{alg:mixematch}
    
    \begin{algorithmic}[1]
        \Require
        \Statex $\mathcal{X} = \big((x_b, y_b); b \in (1, \ldots, B)\big)$,
        \Statex $\mathcal{U} = \big(u_b; b \in (1, \ldots, B)\big)$, $T$, $\alpha$
        
        % \Ensure output

        \Statex
        
        \For{$b \gets 1$ \textbf{to} $B$}
            \State $x^w_{b,1}, {x}^w_{b,2} \gets \text{Aug}^W(x_b, 2)$
            \State $x^s_{b,1}, {x}^s_{b,1} \gets \text{Aug}^S(x_b, 2)$
            \State $u^w_{b,1}, {u}^w_{b,2} \gets \text{Aug}^W(u_b, 2)$
            \State $u^s_{b,1}, {u}^s_{b,1} \gets \text{Aug}^S(u_b, 2)$

            % \Statex
            
            \State ${p}_{b} \gets \frac{1}{2}\big(\mathrm{p}({x}^w_{b,1};\theta, \phi) + \mathrm{p}({x}^w_{b,2};\theta, \phi)\big)$
            \State $\bar{y}_b \gets w_b y_b+(1-w_b){p}_{b}$
            \State ${y}_b \gets \text{Sharpen}(\bar{y}_b,T)$

            % \Statex
            
            \State $\bar{q}_{b} \gets \frac{1}{2}\big(\mathrm{p}({u}^w_{b,1};\theta, \phi) + \mathrm{p}({u}^w_{b,2};\theta, \phi)\big)$
            \State ${q}_{b} \gets \text{Sharpen}(\bar{q}_{b},T)$

            % \Statex
            
            \State ${h}_{x_{b,1}} \gets \mathrm{f}({x}^s_{b,1};\theta)$
            \State ${h}_{x_{b,2}} \gets \mathrm{f}({x}^s_{b,2};\theta)$
            \State ${h}_{u_{b,1}} \gets \mathrm{f}({u}^s_{b,1};\theta)$
            \State ${h}_{u_{b,2}} \gets \mathrm{f}({u}^s_{b,2};\theta)$
         \EndFor
        \Statex

        \State ${\mathcal{X}} \gets \{({x}^s_{b,1},{y}_b), ({x}^s_{b,2},{y}_b);b\in(1,...,B)\}$
        \State ${\mathcal{U}} \gets \{({u}^s_{b,1},q_{b}), ({u}^s_{b,2},q_{b});b\in(1,...,B)\}$
        \State $\mathcal{X}^\prime, \mathcal{U}^\prime \gets \mathopen{} \text{Mixup}({\mathcal{X}}, \mathcal{U}, \alpha)$

        % \Statex
        
        \State ${\mathcal{H}_x} \gets \{({h}_{x_{b,1}},{y}_b), ({h}_{x_{b,2}},{y}_b);b\in(1,...,B)\}$
        \State ${\mathcal{H}_u} \gets \{({h}_{u_{b,1}},q_{b}), ({h}_{u_{b,2}},q_{b});b\in(1,...,B)\}$
        \State $\mathcal{H}_x^\prime, \mathcal{H}_u^\prime \gets \mathopen{}\text{Mixup}({\mathcal{H}_x}, \mathcal{H}_u, \alpha)$

        \Statex

        \State \Return $\mathcal{X}^\prime, \mathcal{U}^\prime, \mathcal{H}_x^\prime, \mathcal{H}_u^\prime$
    \end{algorithmic}
\end{algorithm} 

==> tables/cifar100-v2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\begin{tabular}{llcccc|cccc}
\hline
Corruption                                       & \multicolumn{1}{l|}{}          & \multicolumn{4}{c|}{ImageNet32}                                  & \multicolumn{4}{c}{Places365}                                     \\ \hline
\multicolumn{1}{c}{\multirow{2}{*}{Noise Ratio}} & \multicolumn{1}{l|}{$r_{out}$} & 0.2           & 0.4            & 0.6            & 0.4            & 0.2            & 0.4            & 0.6            & 0.4            \\ \cline{2-10} 
\multicolumn{1}{c}{}                             & \multicolumn{1}{l|}{$r_{in}$}  & 0.2           & 0.2            & 0.2            & 0.4            & 0.2            & 0.2            & 0.2            & 0.4            \\ \hline
\multicolumn{2}{l}{CE}                                                            & 55.52         & 44.31          & 26.03          & 18.45          & 53.61          & 42.46          & 21.42          & 13.85          \\
\multicolumn{2}{l}{M}                                                             & 62.52         & 53.16          & 40.39          & 33.85          & 59.69          & 48.55          & 33.69          & 27.63          \\
\multicolumn{2}{l}{DB}                                                            & 65.61         & 54.42          & 42.5           & 35.9           & 65.83          & 55.61          & 40.61          & 34.86          \\
\multicolumn{2}{l}{JoSRC}                                                         & 64.17         & 61.37          & 37.11          & 41.44          & 66.73          & 60.64          & 39.63          & 32.58          \\
\multicolumn{2}{l}{ELR}                                                           & 68.51         & 63.07          & 44.6           & 34.21          & 68.45          & 62.34          & 36.51          & 33.86          \\
\multicolumn{2}{l}{EDM}                                                           & 70.42         & 61.83          & 14.59          & 1.62           & 70.25          & 61.55          & 14.66          & 11.88          \\
\multicolumn{2}{l}{DSOS}                                                          & 70.54         & 62.05          & 49.14          & 42.88          & 69.12          & 59.47          & 35.41          & 29.48          \\
\multicolumn{2}{l}{RRL}                                                           & 72.33         & 65.44          & 24.51          & 30.64          & 72.49          & 65.79          & 49.27          & 24.34          \\
\multicolumn{2}{l}{SNCP}                                                          & 72.7          & 67.14          & 51.26          & 52.66          & 71.14          & 63.48          & 49.83          & 47.61          \\
\multicolumn{2}{l}{Ours}                                                          & \textbf{75.3} & \textbf{69.08} & \textbf{59.76} & \textbf{62.98} & \textbf{74.54} & \textbf{69.34} & \textbf{58.95} & \textbf{62.46} \\ \hline
\end{tabular}
\end{table*}

==> tables/cifar100-v3.tex <==
\begin{table}[]
 \resizebox{0.5\textwidth}{!}
{%
\begin{tabular}{lcccccccc}
\hline
 % & \multicolumn{8}{c}{Corruption} \\ \cline{2-9} 
 \multicolumn{1}{r}{Corruption}&\multicolumn{4}{c}{ImageNet32} & \multicolumn{4}{c}{Places365} \\ \cline{2-9} 
\multicolumn{1}{c}{$r_{out}$} & 0.2 & 0.4 & 0.6 & 0.4 & 0.2 & 0.4 & 0.6 & 0.4 \\
\multicolumn{1}{c}{$r_{in}$} & 0.2 & 0.2 & 0.2 & 0.4 & 0.2 & 0.2 & 0.2 & 0.4 \\
Method &  &  &  &  &  &  &  &  \\ \hline
CE & 55.52 & 44.31 & 26.03 & 18.45 & 53.61 & 42.46 & 21.42 & 13.85 \\
M & 62.52 & 53.16 & 40.39 & 33.85 & 59.69 & 48.55 & 33.69 & 27.63 \\
DB & 65.61 & 54.42 & 42.5 & 35.9 & 65.83 & 55.61 & 40.61 & 34.86 \\
JoSRC & 64.17 & 61.37 & 37.11 & 41.44 & 66.73 & 60.64 & 39.63 & 32.58 \\
ELR & 68.51 & 63.07 & 44.6 & 34.21 & 68.45 & 62.34 & 36.51 & 33.86 \\
EDM & 70.42 & 61.83 & 14.59 & 1.62 & 70.25 & 61.55 & 14.66 & 11.88 \\
DSOS & 70.54 & 62.05 & 49.14 & 42.88 & 69.12 & 59.47 & 35.41 & 29.48 \\
RRL & 72.33 & 65.44 & 24.51 & 30.64 & 72.49 & 65.79 & 49.27 & 24.34 \\
SNCP & 72.7 & 67.14 & 51.26 & 52.66 & 71.14 & 63.48 & 49.83 & 47.61 \\
Ours & \textbf{75.3} & \textbf{69.08} & \textbf{59.76} & \textbf{62.98} & \textbf{74.54} & \textbf{69.34} & \textbf{58.95} & \textbf{62.46} \\ \hline
\end{tabular}
}
\end{table}

==> tables/redimagnet.tex <==
\begin{table}[t]
    \caption{Web-corrupted miniImageNet from the CNWL~\cite{2020_ICML_MentorMix} ($32\times 32$).  $\star$ shows algorithms using an ensemble of networks to predict and with $\dagger$ algorithms using unsupervised initialization.
    \label{tab:sotamini32}}
    \global\long\def\arraystretch{0.9}%
    \centering
    \resizebox{.6\textwidth}{!}{%
    \centering
    \begin{tabular}{c>{\centering}c>{\centering}c>{\centering}c>{\centering}c>{\centering}c>{\centering}c>{\centering}c>{\centering}c>{\centering}c>{\centering}c}
    \toprule
    Noise level & CE & M & $\star$DM & MM & FaMUS & $\star\dagger$SM & $\star\dagger$PM & DSOS & Ours \tabularnewline
    \midrule
    20 & $47.4$ & $49.1 $ & $51.0$ & $51.0$ & $51.4$ &  $59.1$ & $61.2$ & $61.6$ & $61.4$\tabularnewline
    40 & $42.7$ & $46.4$ & $46.7$ & $47.1$ & $48.0$ & $54.5$ & $56.2$ & $60.0$ &$59.0$\tabularnewline
    60 & $37.3$ & $40.6$ & $43.1$ & $43.8$ & $45.1$ &
    $52.4$ &  $52.8$ & $54.9$ & $ 55.0$ \tabularnewline
    80 & $29.8$ & $33.6$ & $34.5$ & $335$ & $35.5$ & $40.0$ & $43.4$ & $45.6$ & $ $\tabularnewline
       \bottomrule
\end{tabular}}
\end{table}

==> tables/webvision.tex <==
\begin{table}[t]
\caption{Comparison of classification accuracy with the state-of-the-art methods on (mini)Webvision. ``$\star$" denotes algorithms using an ensemble of networks to predict.  All previous works used InceptionResNetV2 model which has about $65$M parameters, while we train PreActResNet-50 which has $25.6$M parameters.
% Results for baseline methods are taken from~\cite{2020_NeurIPS_EarlyReg} and~\cite{albert2022embedding}. MOIT~\cite{2021_CVPR_MOIT} does not evaluate their method on ILSVRC12 as well as did not provide top-5 accuracies.
\label{tab:webvision}}
\centering
\scalebox{1}{
    \begin{tabular}{lcccc} 
        \toprule
         % & \multicolumn{2}{c}{WebVision}\\  \cline{2-3}  
        Method & Top-1 & Top-5 \\ \hline
        Mixup~\cite{2018_ICLR_mixup}& 75.4 & 90.1  \\
        MentrorNet~\cite{2018_ICML_MentorNet} & 63.0 & 81.4 \\
        MentrorMix~\cite{2020_ICML_MentorMix} & 76.0 & 90.2  \\
        $^\star$Co-Teaching~\cite{2018_NeurIPS_CoTeaching}& 63.6 & 85.2  \\
        % Iterative-CV~\cite{2018_CVPR_IterativeNoise} & 65.2 & 85.3 & 61.6 & 85.0 \\
        $^\star$DivideMix~\cite{2020_ICLR_DivideMix} &  77.3 & 91.6  \\
        $^\star$ELR~\cite{2020_NeurIPS_EarlyReg} & 77.8  & 91.7 \\ 
        MOIT~\cite{2021_CVPR_MOIT} & 78.8 & - \\ 
        $^\star$UNICON~\cite{karim2022unicon} & 77.6 & \textbf{93.4}   \\
        ScanMix~\cite{2021_arXiv_Scanmix}& \textbf{80.0}& 93.0  \\
        $^\star$DSOS~\cite{2022_WACV_DSOS}&78.8 & 92.3  \\
        $^\star$PropMix~\cite{2021_arXiv_propmix}& 78.8 & 90.6 \\
        RRL~\cite{2021_ICCV_RRL} & 77.8  & 91.3 \\ 
        SNCP~\cite{albert2022embedding}& 78.2 & 92.6  \\
        \textbf{Ours} &  78.4 & 92.0  \\
        \bottomrule
    \end{tabular}
    }
\end{table}


% \begin{table}[t]
% \caption{Comparison of classification accuracy with the state-of-the-art methods on (mini)Webvision and ILSVRC12. ``$\star$" denotes algorithms using an ensemble of networks to predict. 
% % Results for baseline methods are taken from~\cite{2020_NeurIPS_EarlyReg} and~\cite{albert2022embedding}. MOIT~\cite{2021_CVPR_MOIT} does not evaluate their method on ILSVRC12 as well as did not provide top-5 accuracies.
% \label{tab:webvision}}
% \centering
% % \scalebox{0.9}{
%     \begin{tabular}{lcccc} 
%         \toprule
%          & \multicolumn{2}{c}{WebVision} & \multicolumn{2}{c}{ ILSVRC12}\\  \cline{2-5}  
%         Method & Top-1 & Top-5 & Top-1 & Top-5 \\ \hline
%         Mixup~\cite{2018_ICLR_mixup}& 75.4 & 90.1 & 71.4 & 89.4 \\
%         MentrorNet~\cite{2018_ICML_MentorNet} & 63.0 & 81.4 & 57.8 & 79.9 \\
%         MentrorMix~\cite{2020_ICML_MentorMix} & 76.0 & 90.2 & 72.9 & 91.1 \\
%         $^\star$Co-Teaching~\cite{2018_NeurIPS_CoTeaching}& 63.6 & 85.2 & 61.5 & 84.7 \\
%         % Iterative-CV~\cite{2018_CVPR_IterativeNoise} & 65.2 & 85.3 & 61.6 & 85.0 \\
%         $^\star$DivideMix~\cite{2020_ICLR_DivideMix} &  77.3 & 91.6 & 75.2 & 90.8 \\
%         $^\star$ELR~\cite{2020_NeurIPS_EarlyReg} & 77.8  & 91.7 & 70.3 & 89.8\\ 
%         % MOIT~\cite{2021_CVPR_MOIT} & 78.8 & -  & - & -\\ 
%         $^\star$UNICON~\cite{karim2022unicon} & 77.6 & 93.4 & 75.3 & 93.7  \\
%         % ScanMix~\cite{2021_arXiv_Scanmix}& 80.04& 93.04 &75.76 & 92.60 \\
%         $^\star$DSOS~\cite{2022_WACV_DSOS}&78.8 & 92.3 & 75.9 & 92.4 \\
%         $^\star$PropMix~\cite{2021_arXiv_propmix}& 78.8 & 90.6 & -- & -- \\
%         RRL~\cite{2021_ICCV_RRL} & 77.8  & 91.3 & 74.4 & 90.9\\ 
%         SNCP~\cite{albert2022embedding}& 78.2 & 92.6 & 77.0 & 92.8 \\
%         Ours &  78.4 & 92.0 & \textbf{} & \textbf{} \\
%         \bottomrule
%     \end{tabular}
% \end{table}


% \begin{table}[t]
% \caption{Comparison of classification accuracy with the state-of-the-art methods on (mini)Webvision and ILSVRC12. ``$\star$" denotes algorithms using an ensemble of networks to predict. 
% % Results for baseline methods are taken from~\cite{2020_NeurIPS_EarlyReg} and~\cite{albert2022embedding}. MOIT~\cite{2021_CVPR_MOIT} does not evaluate their method on ILSVRC12 as well as did not provide top-5 accuracies.
% \label{tab:webvision}}
% \centering
% % \scalebox{0.9}{
%     \begin{tabular}{lcccc} 
%         \toprule
%          & \multicolumn{2}{c}{WebVision} & \multicolumn{2}{c}{ ILSVRC12}\\  \cline{2-5}  
%         Method & Top-1 & Top-5 & Top-1 & Top-5 \\ \hline
%         Mixup~\cite{2018_ICLR_mixup}& 75.44 & 90.12 & 71.44 & 89.40 \\
%         MentrorNet~\cite{2018_ICML_MentorNet} & 63.00 & 81.40 & 57.80 & 79.92 \\
%         MentrorMix~\cite{2020_ICML_MentorMix} & 76.00 & 90.20 & 72.9 & 91.10 \\
%         Co-Teaching~\cite{2018_NeurIPS_CoTeaching}& 63.58 & 85.20 & 61.48 & 84.70 \\
%         Iterative-CV~\cite{2018_CVPR_IterativeNoise} & 65.24 & 85.34 & 61.60 & 84.98 \\
%         DivideMix~\cite{2020_ICLR_DivideMix} &  77.32 & 91.64 & 75.20 & 90.84 \\
%         ELR~\cite{2020_NeurIPS_EarlyReg} & 77.78  & 91.68 & 70.29 & 89.76\\ 
%         RRL~\cite{2021_ICCV_RRL} & 77.80  & 91.30 & 74.40 & 90.90\\ 
%         MOIT~\cite{2021_CVPR_MOIT} & 78.76 & -  & - & -\\ 
%         UNICON~\cite{karim2022unicon} & 77.60 & 93.44 & 75.29 & 93.72  \\
%         % ScanMix~\cite{2021_arXiv_Scanmix}& 80.04& 93.04 &75.76 & 92.60 \\
%         DSOS~\cite{2022_WACV_DSOS}&78.76 & 92.32 & 75.88 & 92.36 \\
%         SNCP~\cite{albert2022embedding}&78.26&92.60& 77.00& 92.76 \\
%         % PropMix~\cite{2021_arXiv_propmix}& 78.84&90.56&--& -- \\
%         Ours &  & \textbf{} & \textbf{} & \textbf{} \\
%         % Ours &  78.40& \textbf{92.00} & \textbf{} & \textbf{} \\
%         \bottomrule
%     \end{tabular}
% \end{table}
